Using Focal Loss to Fight Shallow Heuristics: An Empirical Analysis of Modulated Cross-Entropy in Natural Language Inference

There is no such thing as a perfect dataset. In some datasets, deep neural networks discover underlying heuristics that allow them to take shortcuts in the learning process, resulting in poor generalization capability. Instead of using standard cross-entropy, we explore whether a modulated version of cross-entropy called focal loss can constrain the model so as not to use heuristics and improve generalization performance. Our experiments in natural language inference show that focal loss has a regularizing impact on the learning process, increasing accuracy on out-of-distribution data, but slightly decreasing performance on in-distribution data. Despite the improved out-of-distribution performance, we demonstrate the shortcomings of focal loss and its inferiority in comparison to the performance of methods such as unbiased focal loss and self-debiasing ensembles.

==> tables/OLD/exp1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{\textbf{Baseline results.} Comparing the results of our standard configuration with $\gamma=0$ with the numbers we want to reproduce from literature. We match the performance on the MultiNLI validation set and on the HANS constituent heuristic. However, we do not match the performance on the lexical overlap and subsequence heuristics on HANS.}
\label{tab:exp1}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{2}{c}{Heuristic} &  & Lexical overlap & Subsequence & Constituent \\ \midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}HANS Valid\\ Accuracy\end{tabular}} & \multirow{2}{*}{Entailed} & Ours & 0.950 & 0.994 & 0.994 \\ \cmidrule(l){3-6} 
 &  & \cite{mccoy2020berts} & 0.958±0.011 & 0.993±0.004 & 0.990±0.006 \\ \cmidrule(l){2-6} 
 & \multirow{2}{*}{Non-ent.} & Ours & 0.017 & 0.007 & \textbf{0.174} \\ \cmidrule(l){3-6} 
 &  & \cite{mccoy2020berts} & \textbf{0.277±0.124} & \textbf{0.052±0.024} & 0.130±0.041 \\ \midrule[1pt]
\multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MNLI Valid\\ Accuracy\end{tabular}}} & Ours & \multicolumn{3}{c}{0.845} \\ \cmidrule(l){3-6} 
\multicolumn{2}{c}{} & \cite{mccoy2020berts} & \multicolumn{3}{c}{0.843±0.002} \\ \bottomrule
\end{tabular}
}
\end{table}

==> tables/OLD/exp2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\centering
\caption{\textbf{Hyperparameter search for $\gamma=2$}. Hyperparameters are changed one at a time, on top of the standard hyperparameter configuration and $\gamma=2$. The highest overall HANS test performance of 0.508 is achieved by both the standard configuration and the configuration with higher weight decay of $10^{-1}$. \\
Abbreviations: (L)exical overlap, (S)ubsequence, (C)onstituent heuristic; (E)ntailment, (N)on-(E)ntailment.}
\label{tab:exp2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\multicolumn{2}{c}{} & Config & Standard & LR=$2\time10^{-6}$ & LR=$2\time10^{-4}$ & WD=$10^{-3}$ & WD=$10^{-1}$ & BS=$128$ & D=$0.3$ & D=$0.5$ \\ \midrule
\multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MNLI\\ Train\end{tabular}}} & Acc & 0.959 & 0.837 & 0.715 & \textbf{0.989} & 0.977 & 0.890 & 0.863 & 0.780 \\ \cmidrule(l){3-11} 
\multicolumn{2}{c}{} & Loss & 0.031 & 0.148 & 0.278 & \textbf{0.011} & 0.022 & 0.089 & 0.125 & 0.210 \\ \midrule
\multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MNLI\\ Valid\end{tabular}}} & Acc & \textbf{0.846} & 0.830 & 0.355 & 0.843 & 0.842 & 0.845 & 0.842 & 0.800 \\ \cmidrule(l){3-11} 
\multicolumn{2}{c}{} & Loss & 0.391 & \textbf{0.188} & 0.488 & 0.483 & 0.415 & 0.223 & 0.217 & 0.281 \\ \midrule
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}HANS\\ Valid\end{tabular}} & \multirow{2}{*}{All} & Loss & 2.150 & 1.011 & \textbf{0.484} & 2.831 & 2.210 & 1.270 & 1.460 & 0.953 \\ \cmidrule(l){3-11} 
 &  & Acc & {\ul \textbf{0.508}} & 0.488 & 0.500 & 0.500 & {\ul \textbf{0.508}} & 0.500 & 0.495 & 0.490 \\ \cmidrule(l){2-11} 
 & \multirow{3}{*}{E} & L & 0.963 & 0.973 & \textbf{1.000} & 0.961 & 0.967 & 0.980 & 0.973 & 0.980 \\ \cmidrule(l){3-11} 
 &  & S & 0.999 & 0.989 & \textbf{1.000} & 0.979 & 0.994 & 0.998 & \textbf{1.000} & 0.995 \\ \cmidrule(l){3-11} 
 &  & C & 0.997 & 0.969 & \textbf{1.000} & 0.994 & 0.994 & 0.996 & 0.985 & 0.960 \\ \cmidrule(l){2-11} 
 & \multirow{3}{*}{NE} & L & \textbf{0.003} & 0.000 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 \\ \cmidrule(l){3-11} 
 &  & S & \textbf{0.008} & 0.000 & 0.000 & 0.004 & 0.004 & 0.000 & 0.000 & 0.000 \\ \cmidrule(l){3-11} 
 &  & C & 0.077 & 0.000 & 0.000 & 0.057 & \textbf{0.086} & 0.023 & 0.012 & 0.006 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/OLD/exp3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[t]
\centering
\caption{\textbf{Experimental results when varying values of $\gamma$.} The highest overall HANS test performance of 0.523 is reached by the cross-entropy baseline ($\gamma=0$). Increasing $\gamma$ results in worse performance, posing evidence against our hypothesis that focal loss is helpful.}
\label{tab:exp3}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{2}{c}{$\gamma$} &  & 0 & 2 & 5 & 10 \\ \midrule
\multirow{2}{*}{MNLI} & Train & Acc & \textbf{0.980} & 0.959 & 0.959 & 0.880 \\ \cmidrule(l){2-7} 
 & Valid & Acc & 0.845 & \textbf{0.846} & 0.842 & 0.831 \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}HANS\\ Valid\end{tabular}} & Overall & Acc & {\ul \textbf{0.523}} & 0.508 & 0.498 & 0.464 \\ \cmidrule(l){2-7} 
 & \multirow{3}{*}{Entailment} & Lexical & 0.950 & \textbf{0.963} & 0.954 & 0.858 \\ \cmidrule(l){3-7} 
 &  & Subsequence & 0.994 & \textbf{0.999} & 0.992 & 0.950 \\ \cmidrule(l){3-7} 
 &  & Constituent & 0.994 & \textbf{0.997} & 0.992 & 0.961 \\ \cmidrule(l){2-7} 
 & \multirow{3}{*}{Non-entailed} & Lexical & \textbf{0.017} & 0.003 & 0.001 & 0.000 \\ \cmidrule(l){3-7} 
 &  & Subsequence & 0.007 & \textbf{0.008} & 0.002 & 0.000 \\ \cmidrule(l){3-7} 
 &  & Constituent & \textbf{0.174} & 0.077 & 0.050 & 0.017 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/OLD/exp4.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \caption{\textbf{Impact of adding different amount of HANS samples for varying values of $\gamma$.} L, S, and C stand for Lexical overlap heuristic, Subsequence heuristic, and Constituent heuristic, respectively. E and NE stand for Entailment and Non-Entailment. The reported values correspond to the epoch with highest \ac{MNLI} validation accuracy. For $\gamma$=0, i.e. the baseline, the highest overall HANS test performance of 0.523 was reached. Increasing $\gamma$ gave a worse performance, posing evidence against our hypothesis that focal loss will be helpful.}
% \label{tab:exp4}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{ccc|cc|cc|cc|cc|}
% \hline
% \multicolumn{3}{c|}{\# of HANS examples} & \multicolumn{2}{c|}{0} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{1000} & \multicolumn{2}{c|}{10000} \\ \hline
% \multicolumn{3}{c|}{$\gamma$} & \multicolumn{1}{c|}{0} & 2 & \multicolumn{1}{c|}{0} & 2 & \multicolumn{1}{c|}{0} & 2 & \multicolumn{1}{c|}{0} & 2 \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MNLI\\ Acc\end{tabular}} & \multicolumn{2}{c|}{Train} & 0.980 & 0.959 & 0.978 & 0.883 & 0.733 & 0.946 & 0.989 & 0.985 \\ \cline{2-11} 
%  & \multicolumn{2}{c|}{Valid} & 0.845 & 0.846 & 0.847 & 0.845 & 0.844 & 0.844 & 0.847 & 0.845 \\ \hline
% \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}HANS\\ Test\\ Acc\end{tabular}} & \multicolumn{2}{c|}{All} & \textbf{0.523} & 0.508 & \textbf{0.752} & 0.589 & 0.899 & \textbf{0.983} & \textbf{1.000} & \textbf{1.000} \\ \cline{2-11} 
%  & \multirow{3}{*}{E} & L & 0.950 & 0.963 & 0.926 & 0.984 & 0.982 & 0.992 & 1.000 & 1.000 \\ \cline{3-11} 
%  &  & S & 0.994 & 0.999 & 0.947 & 1.000 & 1.000 & 0.998 & 1.000 & 1.000 \\ \cline{3-11} 
%  &  & C & 0.994 & 0.997 & 0.821 & 0.984 & 0.991 & 0.993 & 1.000 & 1.000 \\ \cline{2-11} 
%  & \multirow{3}{*}{NE} & L & 0.017 & 0.003 & 0.552 & 0.154 & 0.807 & 0.963 & 1.000 & 1.000 \\ \cline{3-11} 
%  &  & S & 0.007 & 0.008 & 0.504 & 0.056 & 0.737 & 0.976 & 1.000 & 1.000 \\ \cline{3-11} 
%  &  & C & 0.174 & 0.077 & 0.762 & 0.359 & 0.874 & 0.973 & 1.000 & 1.000 \\ \hline
% \end{tabular}%
% }
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{\textbf{Impact of adding different amounts of HANS training samples when varying values of $\gamma$.} No matter the number of added HANS examples added to the training dataset, cross-entropy consistently outperforms focal loss. Abbreviations: (L)exical overlap, (S)ubsequence, (C)onstituent heuristic; (E)ntailment, (N)on-(E)ntailment.}

\label{tab:exp4}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccc|cc|cc|cc|}
\hline
\multicolumn{3}{c|}{\# of HANS examples} & \multicolumn{2}{c|}{0} & \multicolumn{2}{c|}{100} & \multicolumn{2}{c|}{1000} \\ \hline
\multicolumn{3}{c|}{Gamma} & \multicolumn{1}{c|}{0} & 2 & \multicolumn{1}{c|}{0} & 2 & \multicolumn{1}{c|}{0} & 2 \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MNLI\\ Acc\end{tabular}} & \multicolumn{2}{c|}{Train} & 0.980 & 0.959 & 0.978 & 0.977 & 0.989 & 0.946 \\ \cline{2-9} 
 & \multicolumn{2}{c|}{Valid} & 0.845 & 0.846 & 0.847 & 0.842 & 0.841 & 0.844 \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}HANS\\ Valid\\ Acc\end{tabular}} & \multicolumn{2}{c|}{All} & \textbf{0.523} & 0.508 & \textbf{0.752} & 0.704 & \textbf{0.991} & 0.983 \\ \cline{2-9} 
 & \multirow{3}{*}{E} & L & 0.950 & 0.963 & 0.926 & 0.760 & 0.992 & 0.992 \\ \cline{3-9} 
 &  & S & 0.994 & 0.999 & 0.947 & 0.865 & 1.000 & 0.998 \\ \cline{3-9} 
 &  & C & 0.994 & 0.997 & 0.821 & 0.775 & 0.995 & 0.993 \\ \cline{2-9} 
 & \multirow{3}{*}{NE} & L & 0.017 & 0.003 & 0.552 & 0.452 & 0.978 & 0.963 \\ \cline{3-9} 
 &  & S & 0.007 & 0.008 & 0.504 & 0.569 & 0.989 & 0.976 \\ \cline{3-9} 
 &  & C & 0.174 & 0.077 & 0.762 & 0.803 & 0.995 & 0.973 \\ \hline
\end{tabular}%
}
\end{table}
